OpenGeoBase: Information Centric Networking meets Spatial Database applications - Extended Version

This paper explores methodologies, advantages and challenges related to the use of Information Centric Networking (ICN) for realizing distributed spatial databases. Our findings show that the ICN functionality perfectly fits database requirements: routing-by-name can be used to dispatch queries and insertions, in-network caching to accelerate queries, and data-centric security to implement secure multi-tenancy. We present an ICN-based distributed spatial database, named OpenGeoBase, and describe its design choices. Thanks to ICN, OpenGeoBase can quickly and efficiently provide information to database users; easily operate in a distributed way, deploying and using many database engines in parallel; secure every piece of content; naturally slice resources, so that several tenants and users can concurrently and independently use the database. We also show how OpenGeoBase can support a real world Intelligent Transport System application, by enabling discovery of geo-referenced public transportation information.

==> src/opengeobase-long.tex <==
\section{OpenGeoBase}
\subsection{Offered services}
OpenGeoBase (OGB) is designed to store georeferenced information, i.e. information related to a given spatial area. The database platform is multi-tenant, where a tenant is a principal that rent a slice of storing space. A tenant may use OGB as a database backend for a georeferenced applications. A Tenant has users that, though the application, access OGB data to read or write georeferenced information. OGB read and write access are secured through a data-centric security approach. Users can read and write data only within the slice of their tenant. Users are sure about the owner and the integrity of the georeferenced information they read.        

\subsection{General methodology for ICN Spatial DB}
Spatial databases map the space in an internal data structure to improve the speed up of spatial operations. Such a mapping strategy is also known as indexing methods. In general, an indexing method partitions the space in regions that can be further decomposed in sub-regions. The resulting region hierarchy forms a tree data structure. Most popular indexing methods are Grid, R-Tree, and their variants  \cite{MicrosoftSQL}. 


\begin{figure*}[t]
	\centering
	\subfigure[Grid]{  
		\includegraphics[scale=0.35]{fig/Grid.png}
		\label{f:grid}
	}
	\subfigure[R-tree]{  
		\includegraphics[scale=0.35]{fig/Rtree.png}
		\label{f:rtree}
	}
	\caption{Regions of Grid and R-tree indexing schemes}
	\label{f:indexing}
\end{figure*}


Grid methods , decompose the space into a uniform grid; a tile of the grid can be iteratively split into smaller tiles, realizing a multi-layer hierarchical grid structure; tiles are the nodes of the tree indexing structure \cite{quadtree}; we define \emph{level-ratio} the number of level-$n+1$ tails forming a level-$n$ tail, e.g. level-ratio is 4 in case of fig. \ref{f:indexing}. 
%Range queries can be carried out "tesselating" the requested window with grid tiles and then accessing tiles data. 
%Depending on where spatial objects are actually stored in the indexing tree, a range query could or could not require a recursive resoltion.      
R-trees  decompose the space in overlapping rectangles, whose number, size and position depends on the stored spatial objects, as shown in fig. \ref{f:rtree}. Indeed, spatial objects are enclosed in rectangles; each rectangle is a node of the indexing tree and it is the minimum bounding rectangle that encloses its child rectangles; leaf rectangles contain only one spatial object \cite{guttman1984r}. 
%Range query is carried out using a recursive algorithm: starting from the root node it go down in the tree       


%\emph{Which indexing method does easily fit ICN?} 

\begin{figure*}[t]
	\centering
	\subfigure[Range-query]{  
		\includegraphics[scale=0.30]{fig/range-query.png}
		\label{f:range-query}
	}
	\subfigure[Min stretch tessellationg]{  
		\includegraphics[scale=0.30]{fig/MinStretch.png}
		\label{f:min-streatch}
	}
	\subfigure[Min stretch-and-tiles tessellating]{  
		\includegraphics[scale=0.30]{fig/MinStretch-and-tiles.png}
		\label{f:min-streatch-and-tiles}
	}
	\subfigure[Constrained tessellating ($k=19$)]{  
		\includegraphics[scale=0.30]{fig/constrained.png}
		\label{f:constrained}
	}
	\caption{Range-query and tessellating approaches in case of grid indexing with three levels 0,1,2 and level-ratio 4}
	\label{f:indexing}
\end{figure*}


The general methodology we followed to realize an ICN distributed spatial database consists in assigning unique and routable name prefixes to the regions identified by the indexing process. Each database engine stores data of a subset of regions and exposes the region name-prefixes to the ICN routing plane, e.g. in fig. \ref{f:grid} each level-0 region R$x$ can be assigned to a different engine.  

To resolve a range query, a query-handler function identifies the involved regions through a tessellation procedure and accesses the related spatial data items using the traditional Interest/ContetObject ICN message exchanges. For instance, in fig. \ref{f:min-streatch} the range-query of fig. \ref{f:range-query} is tessellated using a single grid hierarchy. Tessellation procedure returns 42 tiles. After tessellation the query-handler fetches returned tail data through parallel Interest/ContentObject message exchanges (fig. \ref{f:queryhandler}), collects results and send back the range-query response. In our design the query-handler function is provided by the Frontend Library (fig. \ref{f:arch})  
     
%In so doing, we use the ICN routing-by-name functionality as a distributed query dispatcher, achieving a complete horizontal scalability of the system i.e. also the disparcher is distributed. Moreover we use the ICN in-network caching as a query accelerator. 
%\begin{figure}[ht]
%	\centering
%	\includegraphics[scale=0.29]{fig/TesselationConcept.png}
%	\caption{Tesselation process for Grid indexing with three levels 0,1,2. Minimum stretch-and-tiles}
%	\label{f:tesselConcept}
%\end{figure}


\begin{figure}[t]
	\centering
	\includegraphics[scale=0.35]{fig/QueryHandler.png}
	\caption{Range query}
	\label{f:queryhandler}
\end{figure}

To insert a spatial data item, an insert-handler function identifies the involved regions and then push the data item to related engines for storing. Pushing information is not native for ICN architectures such as NDN or CCN, but several solutions actually exists (e.g. \cite{carzaniga2011content} \cite{CCNIOT}, and we propose yet another one but specialized for OpenGeoBase . Delete and Update procedure can follow a similar approach.

In principle, this methodology can be applied both in case of Grid and R-tree indexing. However, we used a grid index since we deemed it to interwork better with ICN technology. Indeed, 
\begin{itemize}
	\item regions of a grid index are unchangeable, i.e. does not depend on the stored objects. Consequently, we can assign unique name-prefixes to them at the system roll out and ICN routing update will be only consequence of administrative reconfigurations, e.g. moving region data from an engine to another one. If regions would be dynamic like in case of R-Tree, at each data insert or removal we risk the introduction of new names in the system and routing plane updates;
	\item  nodes of a Grid indexing tree have a unique parent node, making readily the use of hierarchical naming schemes, in which the name hierarchy reflects the index tree hierarchy. E.g. in fig. \ref{f:grid} the names of level-2 regions of R6 start with R6 prefix. Consequently, the number of routing entries can be dramatically reduced exploiting longest-prefix-matching; e.g. in case an engine handles a region of level-$n$ and all other sub-regions, only a routing entry for the name-prefix of region of level-$n$ is necessary. In case of R-tree a node of the index may have multiple parents and parent may changes over time, thus the use of a hierarchical naming scheme is not straightforward.	
	\item the region-resolution process within query-handler and insert-handler needs to know the shape. Such a knowledge is implicit for Grid methods, and resolution function can be autonomously performed by software libraries running on end devices or application servers. In case of R-tree methods, the region shape is not known a-priori and changes, thus the region-resolution algorithm need to be either updated if run on a single device or realized in a recursive way \cite{du2007sd}, with the drawback of increasing the number of network transmissions involved in the resolution process and query time.
\end{itemize}

\subsection{The Spatial Grid}
The OpenGeoBase spatial grid is a three level grid, aligned with world parallels and meridians, identified by GPS longitude and latitude expressed in decimal degrees, e.g. 12.51133E 41.89193N. A level-0 tile of the grid contains all points having the same longitude and latitude value up to the dot, e.g. the level-0 tile (12,41) contains all points  whose longitude and latitude start with 12 and 41, respectively. A level-$n$ tile of the grid, where $n=1,2$ contains all points having the same latitude and longitude value up to the $n$th decimals, e.g. the level-2 tile (12.51,41.89) contains all points  whose latitude and longitude start with 12.51 and 41.89,respectively. We observe that in so doing each tiles of level-$n$ is formed by 10 tiles of level-$(n+1)$, thus the level-ratio of OpenGeoBase spatial grid is 10. Moreover, for latitude values close to the equator, the area of a level-0 tile approximates a square of 100x100 km, level-1 a square of 10x10 km and a level-2 tile a square of 1x1 km. 

Each level-$n$ tile is identified by a tile-prefix whose structure is:

\texttt{ndn:/OGB/lng(0)/lat(0)/lng(1)lat(1)/ \\ 
	.../lng(n)lat(n)/GPS-ID}

\noindent where lng(0) and lng(k) are the integer and the $k$th decimal value of GPS longitude of the tile. The same relations holds for latitude values.  E.g. the tail (12.51,41.89) has the name prefix ndn:/OGB/12/41/58/19/GPS-ID \footnote{The lng(0) and lat(0) values are decoupled by a slash since they may be composed by different number of characters thus parsing is simpler by separating. Moreover, the decoupling make possible to achieve higher prefix aggregation at routing level}.

%To simplify drawings, in following figures we use spatial grid with level ratio 4 rather than 10.  

\subsection{Range-query Tessellation}
A range-query of an area $A$ is resolved with a set of tile-queries identified by the tessellation procedure. The set $T$ of tiles forming the tessellation cover an area $B$ which contains the area $A$, but also some border additional space, due the fact that the area $A$ may be not aligned with the grid (e.g. see fig. \ref{f:min-streatch-and-tiles}]). We define \emph{tessellation stretch} $TeS$ the ratio between the area $B$ and the area $A$, namely $TeS = area(B)/area(A) \geq 1$.

A \emph{minimum stretch} tessellation is formed by the minimum set of smallest tiles that intersect the area $A$, e.g. level-2 tile as shown in fig. \ref{f:min-streatch}. However, already for small value of $A$ such a computation may returns a lot of tiles, dramatically increasing the overall range-query time. For instance, with smallest tiles of 1 km x 1 km as in case of the OpenGeoBase Spatial Grid, a range query of 50 km x 50 km is tessellated at least with 2500 tiles, i.e. 2500 tile-queries are necessary to satisfy the range-query.  Definitively too much.

To achieve a first reduction of the number of tails, we can merely exploit the hierarchy of the grid, by removing each set of tiles of level $n+1$ that completely cover the parent tile, with such a parent tile of level $n$. This is for instance the case of tessellation reported in fig. \ref{f:min-streatch-and-tiles}, in which a level-1 tails takes place of 4 child level-2 tails and, recursively, a level-0 tail replaces 4 child level-1 tails.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.55]{fig/tesselling.png}
	\caption{Number of tails vs range-query area for minimal stretch-and-tiles tessellation in case of OpenGeoBase spatial grid}
	\label{f:tesseling-perf1}
\end{figure}

However, also this kind of \emph{minimum stretch-and-tiles} tessellation may returns a high number of tails in case of large range-query, e.g. numbers of tiles greater than 500. Indeed, fig. \ref{f:tesseling-perf1} shows the number of tails for randomly centered range-query of square shape, whose area is the x-axis of the plot, using the OpenGeoBase spatial grid. Such high values are usually due to the numerous smallest tiles used to fill the borders of the range-query area and/or to the misalignment of the range-query area with the grid hierarchy.  

Certainly, the number of tiles can be further reduced introducing additional levels in the indexing grid, but each level requires more storage space, how we will discuss in section \ref{s:data-insert}. For this reason, we got the urge to develop a \emph{constrained} tessellation algorithm, in which it is possible to fix the maximum number $k$ of returned tiles. For instance, fig. \ref{f:constrained} show the result of a contrained tesselation for $k=19$. As a drawback, the lower the maximum number of allowed tails, the higher the tessellation stretch $TS$. 

%Starting from the minimum streatch-and-tiles tessellating of 21 tiles in fig. \ref{f:min-streatch-and-tiles}, by imposing a constraint to 19 tiles, 4 tiles of level 2 are replaced by  two tiles of level 1, but as a drawback the tessellated area $B$ and the stretch are greater.

An optimal contrained tesselation algorithm should find the set of $k$ tails providing the minimum stretch. We argue that this problem can be reported to a minimal-weight size-constrained set cover problem. The set $S$ to cover is formed by the set of smallest tiles intersecting the area $A$ and the universe $U$ is formed by these tiles and all their parent tiles up to level-0. The cost of a tile of $U$ is its \emph{tile-stretch}, i.e. the ratio between the tail area and the area of the intersection between the tail area with the range-query area. 

\begin{algorithm} [ht]
	\caption{Constrained Tessellation}
	\label{a:ct}
	%{\fontsize{8}{10}
	\begin{algorithmic}
		\Statex $k$ = max tiles number
		\Statex $n$ = number of levels of the spatial grid
		\Statex $S$ = whole indexing tree
		\Statex $leaf(S)$ = leafs of S, i.e. tiles of the tessellation
		\Statex $MST(S)$ = minimum stretch-and-tiles reduction of $S$
		\Statex
		%\Statex\textit{Tesseling}\
		
		\Statex\textit{constraint violation exception}
		\If {Using all level-0 tiles the number of tiles > $k$}
			
			\Return the set of covering level-0 tiles
		
		\EndIf
		\Statex
		\Statex $S=MST(S)$
				
		\While{number of $leaf(S) > k$}
		
		$i=0$
		
		\While{$i \leq j$}
		\If {(A new level-$i$ tail is necessary)}
		\State Find the new level-$i$ tail with min tail-stretch
		\State Remove all its children from $S$
		\State break
		\EndIf
		
		$i=i+1$
		
		\EndWhile
		\EndWhile\\		
		\Return leaf(S)  
	\end{algorithmic}
	%}
\end{algorithm}

In 2015 the authors of \cite{golab2015size} demonstrate that this problem is NP-hard. According in this paper we devised the simple, but effective, greedy algorithm \ref{a:ct}, which follows a top-down approach by inserting before the necessary bigger tails and then, iteratively, the necessary smaller ones. 

\begin{figure*}[t]
	\centering
	\subfigure[minimum stretch tree]{  
		\includegraphics[scale=0.30]{fig/alg1.png}
		\label{f:alg1}
	}
	\subfigure[minimum stretch-and-tails tree]{  
		\includegraphics[scale=0.30]{fig/alg2.png}
		\label{f:alg2}
	}
	\subfigure[A level 0 tiles inserted since necessary]{  
		\includegraphics[scale=0.30]{fig/alg3.png}
		\label{f:alg3}
	}
	\subfigure[A level 1 tiles inserted since necessary]{  
		\includegraphics[scale=0.30]{fig/alg4.png}
		\label{f:alg4}
	}
	\caption{Constrained tessellation with max-tiles $k$ = 6 in case of a three level grid (0,1,2) with level-ratio 4. Dark circle are the leafs nodes forming the tessellation}
	\label{f:alg}
\end{figure*}

We explain the algorithm following the example in fig. \ref{f:alg}, in which max-tails constraint is $k=6$. We start from the minimum stretch indexing tree containing all the level-2 tiles intersecting the range-query area and all related parents up to level-0. Dark circles are the leaf nodes of the tree and forms the tessellation set $T$. The tile-stretch value is reported inside the circles. We assume that with this configuration the tessellation stretch $TeS$ is equal to 1, i.e. the range query area is aligned with the level-2 grid.  Then, in fig. \ref{f:alg2} we readily derive the minimal stretch-and-tail (MST) tree by pruning all leafs of nodes that have all the children (4 in this case). 

Now we observe that to respect the constraint $k=6$, we need to insert in the tessellation a new tile of level-0, i.e. to remove from the tree all children of such a tile. In general, a level-$i$ tail is necessary  when also inserting in the tessellation all the remaining level-$i+1$ tiles we would not be able to respect the constraint. Thus a level-$i$ "aggregation" is surely necessary.  
%if pruning all child nodes of the level-$i+1$ non-leaf nodes, the resulting tree has a number of leafs greater than $k$.
%In our case, inserting in the tessellation all the six remaining level-1 tiles, we would get a tessellation with 8 tiles (a tree with 8 level-1 leafs), thus a level-0 tile must be inserted in the tessellation. 
Following a greedy approach, we single out the level-0 tile with the minimum tile-streth, i.e. 1.45, and obtain the tree in fig. \ref{f:alg3}. 

In next iteration a new level-0 tiles is not necessary, but a new level-1 tile is. We randomly chose one of the two level-1 tiles with minimum tile-stretch 2 and obtain the tree in fig. \ref{f:alg4}, whose 6 leafs form the constrained tessellation and provide an overall tessellation stretch of 27/20: 20 is the number of level-2 tiles perfectly matching the range-query area $A$ and 27 is overall number of level-2 tiles belonging to the tessellated area $B$.                


This algorithm is surely not optimal because, using a brute-force search of the optimal solution, we find some extremely rare cases in which the algorithm solution is not the mimimum streatch one. In any case, the finding of the optimal constrained tessellating is out of the scope of this paper. Here, we merely wish to put forward the existence of problem and a simple solution.
  
  
\begin{figure}[t]
 	\centering
 	\includegraphics[scale=0.55]{fig/tesseling-stretch.png}
 	\caption{Stretch of constrained tessellation vs range-query area in case of OpenGeoBase spatial grid}
 	\label{f:tessellating-strech}
\end{figure}

Fig. \ref{f:tesseling-perf1} show that the constrained tessellating algorithm is actually able to reduce the number of query up to the constraint $k=100$. Fig. \ref{f:tessellating-strech} reports the drawback of limiting the maximum number of tails, i.e. an increase of the tessellation stretch $TeS$. Roughly, using 100 tiles we achieve have a streach about of 50\% for very large query-areas, such as 50,000 km$^2$. Using 200 and 400 tiles this value fall down to 22\% and 10\%, respectively \footnote{We observe that also in case of the unconstrained minimal stretch-and-tails solution there is a little stretch due to the fact that we can not have a resolution lower than the smaller grid level; however stretch value are extremely close to one}.          

Having a stretch greater than 1 implies that a range-query would obtain data related to a greater area, thus possibly more data than necessary ones, which can be filtered out at the application end. Accordingly, on the one hand, reducing the number of tails we are reducing the range-query processing time since less tail-queries are required, but on the other hand we are increasing the transmission time since transferred data may be more. Clearly a trade off is in the order; which depends on the density and volume of georeferenced information. And such values are application dependent.       

\subsection{Data structures}
OpenGeoBase handles three kinds of data structure, namely: \emph{OGB-Data}, \emph{OGB-Tail} and \emph{OGB-IP-Resolution}
An OGB-Data is a georeferenced information associated to a tile of the grid. It resembles a <key,value> tupla, where the key uniquely identifies the belongings tile. For instance, <(12.51,41.89) , [Starbucks]> could mean that a Starbucks coffee is within the tile (12.51,41.89). If the finest tile level localization (1 km x 1 km) would be too coarse, precise GPS coordinates may be inserted in a field of the value and processed by the application, e.g. a value structure may be [12.51133:41.89193, Starbucks]. To exploit ICN, an OGB-Data is exactly a ContentObject, whose name includes the key, and whose content is the value. Specifically, the OGB-Data naming scheme is:

\texttt{ndn://tile-prefix/DATA/tenant-id/app-dep /user-id}

\noindent where tenant-id is the identifier of the Tenant slice in which the OGB-Data is stored, user-id is the user identifier and app-dep are intermediate application dependent name components; e.g. in case of a Point of Interest (POI) application the app-dep scheme may be POI-type/POI-name.

To solve a range query a receiver should download all OGB-Data items contained in the tails, identified by the tesselation process. Since a tail may contain several OGB-Data, to accelerate a tail-query we defined the OGB-Tail structure as a container of all the OGB-Data items of a tile. From the ICN point of view, OGB-Tail is a single ICN content with a unique name, in case properly segmented by the plain ICN/NDN segmenter \cite{ndn}. Using OGB-Tail we are able to satisfy a single tile-query with a two-ways, query-response, handshake and reduce latency, with respect to a much more naive, 4-ways, approach of answering the tile-query with the list of OGB-Data names and then fetching these OGB-Data items one by one.
The OGB-Tail naming scheme is:

\texttt{ndn://tile-prefix/TAIL/tenant-id}  

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.30]{fig/DataStructures.png}
	\caption{OGB-Data, OGB-Tail (no segmentation) and OBG-IP-Resolution structures }
	\label{f:datastructure}
\end{figure}


Fig. \ref{f:datastructure} report a case for which a OpenGeoBase 100x100 tail with lng=12 and lat=41 with tenant-id is Foo contains two georeferenced information, i.e. two OGB-Data ContentObjects: one of Alice and one of Bob. When queried for this tile the database engine sends back the OGB-Tile whose content is the collection of the two OGB-Data ContentObjects. In fig. \ref{f:queryhandler}, the tail-data are actually OGB-Tail.

OGB-Tail are cached by ICN nodes thus popular tail-queries can be quickly satisfied  from the cache. To avoid the presence of stale data in the cache, the FreshnessPeriod of the OGB-Tail ContetObjects can be properly configured by the tenant. Otherwise, if a more reactive cache update approach is needed new network mechanism should be introduced.    

The third data structure is the OGB-IP-Resolution. It is a ContentObject used to derive the IP address of the database engine handling a given tile-prefix. The name used for an OGB-IP-Resolution has the following scheme:

\texttt{ndn://tile-prefix/IP-RES/tenant-id}
\noindent and its use will be discusses in next section \ref{s:data-insert}     

\subsection{Data Insert}
\label{s:data-insert}
To insert a georeferenced tile am insert-handler function has to create and push the related OGB-Data to the responsible database engine.  

If the ICN architecture provided data push services, the data insert procedure would be trivial: the insert-handler would feed the ICN network layer with the OGB-Data and the ICN routing plane would route by name this message towards the responsible database engine, like it occurs for routing Interests of tail-queries.      

But ICN architectures such as NDN and CCN natively offer data pull services and, honestly, to realize to push data using NDN/CCN is a little more complex, with respect to push data using TCP/IP. Clearly, this is not a NDN/CCN lack, rather a precise design choice considering that the most of Internet applications are pull-based.      

More complex but not impossible, indeed several literature proposals describe methods to push data over NDN/CCN. A typical solution provides that a produced send an initial Interest versus the consumer to solicit it to pull the producer data, thus realizing an Interest-Interest-ContentObject three-way handshake  for push one data. 

It is worth to note that this approach requires a routable producer prefix through the which consumer can pull sender data. 
%But when producers are (mobile) end-users, supporting routable prefixes towards them may creates security and scalability problem at the routing plane. 
And in our database application this would imply to set up an NDN route towards end user applications requiring data insert. In doing so, we would give to these applications the critical power to impact network-layer routing plane, paving the way to potential security and scalability problems. For this reason we deemed this approach not suitable for our scenario. 
%And in any case route setup may further increase the insert delay beyond the three-way handshake.

Other push approaches \cite{franccois2013ccn}\cite{carzaniga2011content} provide to change the NDN/CCN FIB operation to route push-data by name, using the same FIB forwarding procedures used for Interest messages. These approaches are fast, since realize data push with a one-way interaction, like IP does. But they require a change of current NDN/CCN implementations, that currently we prefer to avoid.    

Since up to know we did not find a data push solution suitable for our application (i.e. secure, scalable, no-change of NDN software), we devised a new one getting the inspiration from a little known procedure available in the NDN software, namely \emph{TCP-bulk-insert}. Using TCP-bulk-insert a producer sets up a TCP socket with a data repository (consumer) for transferring one or more ContentObject. The repository can check ContentObjects' validity before storing them. Albeit this is not a "pure" ICN procedure, we consider this mechanism very effective to push ContentObject towards a single consumer, that is exactly our use case: push one or more OGB-Data towards the responsible database engine. 

But to use the TCP bulk insert we need to know the IP address of the database engine. And this IP address may change when system administrator decide to relocate spatial regions among databases, e.g. in case of an horizontal scaling. Accordingly, we devised a simple ICN-based  IP address resolution procedure that use the OGB-IP-Resolution data structure previously presented. 

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.30]{fig/datainsert.png}
	\caption{Data Insert}
	\label{f:datainsert}
\end{figure}

Overall, fig. \ref{s:data-insert} shows the data-insert procedure. The insert-handler receives a georeferenced information. Computes associated the tile(s) and prepare the related OGB-Data. Then resolve the IP address of the database responsible of the tile sending an Interest for the OGB-IP-Resolution content. The databalse receive that Interest and sends back the ContetObject whose content is its IP address. The insert-handler setup the TCP socket and transfer the OGB-Data.

The computation of the tiles associated to a georeferenced information should take into account that a range-query procedure can autonomously choose tiles of any level. This implies that a georeferenced information has to be stored in the containing tile of any level. We call this methodology as \emph{level-replication}. E.g. using the OpenGeoBase spatial grid, a point of interest should be embedded in three different OGB-Data, related to the 1x1, 10x10 and 100x100 containing tiles. Consequently, the more the levels, the more the storage space required to store an information.  

A traditional approach to avoid storage replication is to insert actual data only on the leaf node of the indexing grid (1x1 tiles), and to insert only links to data in the higher level tiles. However, in doing so either we avoid the possibility of horizontally scale grid levels in different database, or we need resolve a tail-query through a network iteration \cite{du2007sd} with an increase of the range-query time. And since we wish to speed up range-query as much as possible, we retained this solution not suitable and to pay speed with storage space. Nevertheless, we hope to find in the future a more storing space conservative approach. 

It is wort to point out that level-replication is not always strictly necessary, but it is application dependent. Indeed, there are some applicants for which the georeferenced information can be aggregated with the observation scale. In these cases, only a single aggregated value per level is necessary. For instance, to realize an application showing the number of lions in a given region, we need to store the number of lions in each 1x1 tiles. Then, for each 10x10 tiles we need to store only one data: the sum of the values of the child 1x1 tiles.       

\subsection{Database Engine}
A database engine process tail-queries expressed with Interest of OBG-Tail contents and store georeferenced data in the form of OGB-Data ContetObjects. To desing the engine we extended the actual NDN Repo-ng \cite{ndn} which is formed by: a frontend module that process Interest messages and TCP bulk inserts; and a  backend database management system (DBMS) where to SELECT and INSERT ContetObjects. The default DBMS of NDN Repo-ng is SQLite \cite{sqlite} and contain a single table (CO-Table), whose rows contains the stored ContentObjects. 

We extend Repo-ng in order to handle and speed-up the processing of OBG-Tail Interest messages, i.e. tail-queries. We added three tables to the Repo-ng DBMS, named, Tile-Tables, one per OpenGeoBase Spatial Grid level. The rows of the tile-table of level $i$ contain the names of OGB-Data ContentObjects belonging to any tile of level $i$. 

When an OBG-Tail Interest for a tail $x$ of level $i$ is received, the frontend performs an SQL SELECT on the rows of tile-table of level $i$, searching for those names whose prefix is equal to the prefix of tail $x$. To speed-up this string matching we used the XXXXXXX module of sqlite3. And having different tables per level we are reducing the search space thus the query processing time. Clearly, other possible table designs are possible, but again here we wish to put forward the problem rather that find the best solution. The SQL SELECT returns to the frontend the names of ContetObjects that are fetched from the CO-Table and sent back to the Application through an NDN segmenter.  

We also modified the TCP bulk insert procedure so as to create related rows of tile-tables.                      


\subsection{Security}
NDN security library make possible to sign Interests and ContentObjects and insert the name of the certificate to be used to verify the sign, namely KeyLocator, so that any device can fetch it from NDN, if unavailable locally. 
A NDN certificate includes the identity name of the owner, its public key, the sign of the certification authority and the KeyLocator of certification authority.  When an Interest or a ContetObject is received it can be validated using a Validator tool whose trust schema \cite{ndntrust} can be flexibly configured using rules and trust-anchors. 

To support OpenGeoBase multi-tenancy we exploited NDN security library as is, thus we do not describe many details. The trust chain provides that the user of a tenant have a unique identity released by the tenant and the tenant signs and releases user certificates. Tenant identity is provided by the administrator of the system that also releases and signs its certificates. The public key of the system administrator is the trust anchor. 

A OGB-Tiles Interest message related to a tile of a tenant are signed by the message issuer. Tenant identity is included in the OGB-Tile name. Using a proper configuration of the Validator and of KeyLocator names, edge NDN nodes or directly database engines if no other kind of NDN nodes exist in the backend (our case), accepts only OGB-Tiles Interest message whose certificate of the issuer has been released by the tenant of the tile. 
%In doing so, tail-query regarding data of a tenant slice are processed only if the issuer is a user of the same tenant.

A OGB-Data ContentObject is signed by the data owner. Owner identity is included in the OGB-Data name. This makes possible to properly configure the Validator of the query-handler so as verifying that the OGB-Data related to an owner is actually signed by the owner. Dually, it is possible to configure the Validator of the database engine to insert only OGB-Data ContentObjects whose identity contained in the name is the same of the owner of the signing certificate. A OGB-Tile and OGB-IP-Resolution ContentObjects are signed by the system administrator.

%We observe that using such a configuration to speed-up query and insert security checks the database engines should have the certificates of all the users in their certificate store. Indeed, retrieving remotely at run time the certificate using KeyLocator may dramatically delay query and insert processing.          
                           

\subsection{Bloom Pre-filtering}
When georeferenced information are rather sparse, many of the tessellated tail-queries are void and thus the related OGB-Tail Interest either goes in timeout or, as in our case, is followed by a void ContetObject since timeout elapsing may get a longer time. A classical approach to avoid useless queries is the use Bloom Filters \cite{broder2004network} for pre-filtering the query set before actually submit the queries to the database engines. Also OpenGeoBase uses this approach. OpenGeoBase Bloom Filter (BF) is loaded with name prefixes of tails that are not void. After the tessellation, the query-handler test the BF membership of tessellated tiles and obtain a reduced set tessellation comprising only not void tiles. 

Georeferenced information contained in the database can change frequently. consequently, the BF can not be distributed to the query-handlers since the synchronization effort could be overwhelming, considering that query-handlers can also run within end-devices. For this reason, the OpenGeoBase architecture contains one or more BF servers that handles membership requests, as show in fig. \ref{f:queryhandler}. The price to pay is an additional RTT in the range-query time. And the price worth only when geo-referenced data are rather sparse, thus the use of BF is left optional up to the tenant.

To update the BF we use a publish-subscribe approach \cite{chen2011copss}. Each database engine has a Counting Bloom Filter (CBF) with the same buckets of the BF running on the server. At each data insert/removal the CBF is updated. When a bucket becomes greater than zero or becomes equal to zero a publication is sent out. The BF server is a subscriber of such publications. 
                       
Currently, we have not yet implemented the publish-subscribe infrastructure, but are going to use the one we proposed in \cite{detti2015exploiting} merely because does not requires any NDN changes. 
   
   

